ConvoSumm: Conversation Summarization Benchmark and Improved Abstractive Summarization with Argument Mining

While online conversations can cover a vast amount of information in many different formats, abstractive text summarization has primarily focused on modeling solely news articles. This research gap is due, in part, to the lack of standardized datasets for summarizing online discussions. To address this gap, we design annotation protocols motivated by an issues--viewpoints--assertions framework to crowdsource four new datasets on diverse online conversation forms of news comments, discussion forums, community question answering forums, and email threads. We benchmark state-of-the-art models on our datasets and analyze characteristics associated with the data. To create a comprehensive benchmark, we also evaluate these models on widely-used conversation summarization datasets to establish strong baselines in this domain. Furthermore, we incorporate argument mining through graph construction to directly model the issues, viewpoints, and assertions present in a conversation and filter noisy input, showing comparable or improved results according to automatic and human evaluations.

==> old/0-save_helpers.tex <==

% Section 3
\newcommand{\DatasetComparison}{
 \begin{table*}[t!]
\resizebox{\textwidth}{!}{\begin{tabular}{c c c c c c}
\Xhline{2\arrayrulewidth}
             \textbf{Dataset} & \textbf{\% novel n-grams} & \textbf{Extractive Oracle}  &  \textbf{Summary Length} & \textbf{Input Length}  & \textbf{\# Docs/Example} \\  \hline
            NYT & 36.11/79.72/94.52 & 36.26/10.21/31.23 & 79 & 1624 & 16.95  \\ \hline  
            Reddit & 43.84/84.98/95.65 & 35.74/10.45/30.74  & 65 & 641 & 7.88 \\ \hline  
            Stack & 35.12/77.91/93.56 &  37.30/10.70/31.93  & 73 & 1207 & 9.72   \\ \hline  
            Email & 42.09/83.27/93.98 & 40.98/15.50/35.22  & 74 & 917 & 4.95  \\ \hline  
            \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Statistics across dataset sources in ConvoSumm, showing novel uni/bi/tri-grams, ROUGE-1/2/L extractive oracle scores, the average input and summary lengths (number of tokens), as well as the number of documents per example, where each comment/post/answer/email is considered a document.}
\label{tab:statistics}
\end{table*}
}

\newcommand{\DatasetComparisonMDS}{
 \begin{table}[t]
\resizebox{\columnwidth}{!}{\begin{tabular}{c c c c c c}
\Xhline{2\arrayrulewidth}
             \textbf{Dataset/Method} & \textbf{Inter-document Similarity} & \textbf{Redundancy} & \textbf{Layout Bias} \\  \hline
            NYT & -11.71 & -0.23 & 0.2/0.5/0.3  \\ \hline  
            Reddit & -7.56 & -0.49 & 0.2/0.5/0.2  \\ \hline  
            Stack & -9.59 & -0.27 & 0.2/0.3/0.4 \\ \hline  
            Email & -1.76 & -0.18 & 0.3/0.4/0.3 \\ \hline  
            \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Multi-document summarization-specific dataset analysis on our proposed datasets with metrics introduced in \citet{dey2020corpora}:   inter-document similarity (father from zero is less similarity), redundancy (father from zero is less overall redundancy of semantic units), and start/middle/end layout bias.}
\label{tab:statistics_mds}
\end{table}
}

\newcommand{\BaselineResults}{
 \begin{table}[t]
\resizebox{\columnwidth}{!}{\begin{tabular}{c c c c}
\Xhline{2\arrayrulewidth}
             \textbf{Dataset/Method} & \textbf{Lexrank} &  \textbf{Textrank} & \textbf{BERT-ext} \\  \hline
            NYT & 22.30/3.87/19.14 & 25.11/3.75/20.61 & 25.88/3.81/22.00  \\ \hline  
            Reddit & 22.71/4.52/19.38 & 24.38/4.54/19.84 & 24.51/4.18/20.95 \\ \hline  
            Stack & 26.30/5.62/22.27 & 25.43/4.40/20.58 & 26.84/4.63/22.85 \\ \hline  
            Email & 16.04/3.68/13.38 & 19.50/3.90/16.18 & 25.46/6.17/21.73 \\ \hline  
            \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{ROUGE-1/2/L results for extractive LexRank \cite{erkan2004lexrank}, TextRank \cite{mihalcea2004textrank}, and BERT-based \cite{miller2019leveraging} models.}
\label{tab:extractive_baselines}
\end{table}
}


% % Section 5
\newcommand{\BARTTransferResults}{
 \begin{table}[t]
\resizebox{\columnwidth}{!}{\begin{tabular}{| c | c |  c |}
\Xhline{2\arrayrulewidth}
             \textbf{Data/Method}  &  \textbf{BART} & \textbf{BART-arg} \\  \hline
            NYT &  35.91/9.22/31.28 & \textbf{36.60}/ \textbf{9.83}/\textbf{32.61} \\ \hline  
            Reddit &  35.50/10.64/32.57 & \textbf{36.39}/ \textbf{11.38}/\textbf{33.57}  \\ \hline  
            Stack &  39.61/10.98/35.35 & \textbf{39.73}/ \textbf{11.17}/\textbf{35.52}  \\ \hline  
            Email &  \textbf{41.46}/\textbf{13.76}/ \textbf{37.70} & 40.91/13.67/37.10   \\ \hline  
            \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{ROUGE-1/2/L results for vanilla BART as well as one trained on argument-mining input. Both are trained on 200 points from the ConvoSumm.}
\label{tab:bart_transfer}
\end{table}
}

% Section 6
\newcommand{\BARTMeetingResults}{
 \begin{table}[t]
\resizebox{\columnwidth}{!}{\begin{tabular}{c c c c c}
\Xhline{2\arrayrulewidth}
             \textbf{Dataset/Method} & \textbf{HMNet}  &  \textbf{DDA-GCN}  &  \textbf{Longformer-BART} & \textbf{Longformer-BART-arg} \\  \hline
            AMI &  53.02/18.57/- & 53.15/\textbf{22.32}/- & 54.20/20.72/51.36   &  \textbf{54.47}/20.83/\textbf{51.74} \\ \hline  
            ICSI & \textbf{46.28}/10.60/- & -  & 43.03/\textbf{12.14}/40.26 & 44.17/11.69/\textbf{41.33}  \\ \hline  
            \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{ROUGE-1/2/L results for DDA-GCN \cite{feng2020dialogue} and HMNet \cite{zhu2020a} on the AMI and ICSI meeting summarization dataset along with our Longformer and Longformer-arg models.}
\label{tab:meeting}
\end{table}
}

\newcommand{\TableHumanEvaluation}{
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{c | c c |  c c} \Xhline{2\arrayrulewidth}
            \textbf{Target Dataset} &  \multicolumn{2}{c|}{BART} &  \multicolumn{2}{c}{BART-arg}  \\
              &  Relevance & Consistency & Relevance & Consistency \\
          \Xhline{2\arrayrulewidth} 
          Reddit   &  3.39 & 3.40 &  3.47 &  3.41 \\
          AMI   &  4.07 & 3.67 &  4.13 &  3.70 \\
            \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Relevance and factual consistency annotations for BART and BART-arg outputs on Reddit and AMI.}
\label{tab:table_human_evaluation}
\end{table}
}



\newcommand{\BARTBenchmarkOthers}{
 \begin{table}[t]
\resizebox{\columnwidth}{!}{\begin{tabular}{c c c}
\Xhline{2\arrayrulewidth}
             \textbf{Dataset/Method} & Our results  &  Previous SOTA \\  \hline
            SAMSum & \textbf{52.27/27.82/47.92} & 49.30/25.60/47.70   \\ \hline   
            CQASUMM  & \textbf{32.79/6.68/28.83} & 31.00/5.00/15.20   \\ \hline  
            BC3 & 39.59/13.98/21.20 & -   \\ \hline  
            ADS & 37.18/11.42/21.27 & -   \\ \hline  
            SENSEI & 34.57/7.08/16.80 & -   \\ \hline  
            \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Benchmarking results on conversational datasets such as SAMSum \cite{gliwa-etal-2019-samsum} and CQASUMM \cite{chowdhury2018cqasumm} and initial neural abstractive summarization results for email (BC3) \cite{JanAAAI08}, debate discussion forums (ADS) \cite{misra-etal-2015-argumentative-dialogue-corpus}, and news comments (SENSEI) \cite{barker2016sensei}.}
\label{tab:benchmark_others}
\end{table}
}






==> old/0-save_helpers_backup.tex <==


% % Section 1
% \newcommand{\IntroductionMotivatingExample}{
% \begin{table}[t!]
% \centering
% \small
% \begin{tabularx}{\columnwidth}{|X|}
% \hline
% \textbf{Headline:} SuperBowl
%  \\ \hline
% \textbf{Snippet:} Whether you’re a football fan or not, what do you like about Super Bowl Sunday?
%  \\ \hline
% \textbf{Comment:} ... In my opinion I think the Falcons will stomp the patriots. I think Tom Brady will choke the Super Bowl. ...
% \\ \hline
% \textbf{Comment:}  I am big Arizona Cardinals fan so when they didn't even make the playoffs i was upset. ...
% \\ \hline
% \textbf{Comment:} I'm not a very big football fan at all. So when it comes to Superbowl Sunday, I'm in it for the commercials and the half time show. ...
% \\ \hline
% \textbf{Comment:}  I am not exactly a football fan, but I enjoy watching the Super Bowl....
% \\ \hline
% \textbf{...}
% \\ \hline
% \textbf{Summary:} \\ 
% Several commenters list their favorite things about the Super Bowl, including half-time shows, the funny commercials, the Puppy Bowl, eating food, and spending time with family. A couple of commenters admit to not being football fans but still enjoying the Super Bowl. Some commenters discuss whether they thought the Falcons or the Patriots were going to win, while others list teams they wish were in the game.
%  \\
% \hline
% \end{tabularx}
% \caption{Example summary of comments from a New York Times article discussing people's favorite parts of the Super Bowl. The summary is an analysis of the comments and quantifies the viewpoints present.}
% \label{tab:example}
% \end{table}
% }

% % Section 3
% \newcommand{\DatasetComparison}{
%  \begin{table*}[t!]
% \resizebox{\textwidth}{!}{\begin{tabular}{c c c c c c c c c c}
% \Xhline{2\arrayrulewidth}
%              \textbf{Dataset} & \multicolumn{3}{c}{\textbf{\% novel n-grams}} &  \multicolumn{3}{c}{\textbf{Extractive Oracle}}  &  \textbf{Summary Length} & \textbf{Input Length}  & \textbf{\# Docs/Example} \\  \hline
%             NYT & 36.11 & 79.72 & 94.52 & 36.26 & 10.21 & 31.23 & 79 & 1624 & 16.95  \\ \hline  
%             Reddit & 43.84 & 84.98 & 95.65 & 35.74 & 10.45 & 30.74  & 65 & 641 & 7.88 \\ \hline  
%             Stack & 35.12 & 77.91 & 93.56 &  37.30 & 10.70 & 31.93  & 73 & 1207 & 9.72   \\ \hline  
%             Email & 42.09 & 83.27 & 93.98 & 40.98 & 15.50 & 35.22  & 74 & 917 & 4.95  \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Statistics across dataset sources in ConvoSumm, showing novel uni/bi/tri-grams, ROUGE-1/2/L extractive oracle scores, the average input and summary lengths (number of tokens), as well as the number of documents per example, where each comment/post/answer/email is considered a document.}
% \label{tab:statistics}
% \end{table*}
% }
% \newcommand{\DatasetComparisonMDS}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{c c c c c c}
% \Xhline{2\arrayrulewidth}
%              \textbf{Dataset/Method} & \textbf{Inter-document Similarity} & \textbf{Redundancy} & \textbf{Layout Bias} \\  \hline
%             NYT & -11.71 & -0.23 & 0.2/0.5/0.3  \\ \hline  
%             Reddit & -7.56 & -0.49 & 0.2/0.5/0.2  \\ \hline  
%             Stack & -9.59 & -0.27 & 0.2/0.3/0.4 \\ \hline  
%             Email & -1.76 & -0.18 & 0.3/0.4/0.3 \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Multi-document summarization-specific dataset analysis on our proposed datasets with metrics introduced in \citet{dey2020corpora}:   inter-document similarity (father from zero is less similarity), redundancy (father from zero is less overall redundancy of semantic units), and start/middle/end layout bias.}
% \label{tab:statistics_mds}
% \end{table}
% }
% \newcommand{\BaselineResults}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{c c c c}
% \Xhline{2\arrayrulewidth}
%              \textbf{Dataset/Method} & \textbf{Lexrank} &  \textbf{Textrank} & \textbf{BERT-ext} \\  \hline
%             NYT & 22.30/3.87/19.14 & 25.11/3.75/20.61 & 25.88/3.81/22.00  \\ \hline  
%             Reddit & 22.71/4.52/19.38 & 24.38/4.54/19.84 & 24.51/4.18/20.95 \\ \hline  
%             Stack & 26.30/5.62/22.27 & 25.43/4.40/20.58 & 26.84/4.63/22.85 \\ \hline  
%             Email & 16.04/3.68/13.38 & 19.50/3.90/16.18 & 25.46/6.17/21.73 \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{ROUGE-1/2/L results for extractive LexRank \cite{erkan2004lexrank}, TextRank \cite{mihalcea2004textrank}, and BERT-based \cite{miller2019leveraging} models.}
% \label{tab:extractive_baselines}
% \end{table}
% }


% % Section 4
% \newcommand{\ArgumentGraph}{
% \begin{figure*}[t!]
%     \centering
%     \includegraphics[scale=0.40]{plots/argument_graph.png}
%     \caption{Sample argument subgraph construct from NYT news comments illustrating varying viewpoints. Claims "I honestly..." and "but I dont.." are entailed by premises, connected through \texttt{Default Inference} nodes, and opposing claims are connected through \texttt{Issue} nodes.
%     }
%     \label{fig:argument_graph}
% \end{figure*} 
% }


% % Section 5
% \newcommand{\BARTTransferResults}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{c c c}
% \Xhline{2\arrayrulewidth}
%              \textbf{Dataset/Method}  &  \textbf{BART} & \textbf{BART-arg} \\  \hline
%             NYT &  35.91/9.22/31.28 & \textbf{36.02/9.60/32.34} \\ \hline  
%             Reddit &  35.50/10.64/32.57 & \textbf{36.39/11.38/33.57}  \\ \hline  
%             Stack &  39.61/10.98/35.35 & \textbf{39.73/11.17/35.52}  \\ \hline  
%             Email &  \textbf{41.46/13.76/37.70} & 40.91/13.67/37.10   \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{ROUGE-1/2/L results for vanilla BART as well as one trained on argument-mining input. Both are trained on 200 points from the ConvoSumm.}
% \label{tab:bart_transfer}
% \end{table}
% }


% % Section 6
% \newcommand{\BARTMeetingResults}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{c c c c c}
% \Xhline{2\arrayrulewidth}
%              \textbf{Dataset/Method} & \textbf{HMNet}  &  \textbf{DDA-GCN}  &  \textbf{Longformer-BART} & \textbf{Longformer-BART-arg} \\  \hline
%             AMI &  53.02/18.57/- & 53.15/\textbf{22.32}/- & 54.20/20.72/51.36   &  \textbf{54.47}/20.83/\textbf{51.74} \\ \hline  
%             ICSI & \textbf{46.28}/10.60/- & -  & 43.03/\textbf{12.14}/40.26 & 44.17/11.69/\textbf{41.33}  \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{ROUGE-1/2/L results for DDA-GCN \cite{feng2020dialogue} and HMNet \cite{zhu2020a} on the AMI and ICSI meeting summarization dataset along with our Longformer and Longformer-arg models.}
% \label{tab:meeting}
% \end{table}
% }

% \newcommand{\TableHumanEvaluation}{
% \begin{table}[t!]
% \centering
% \resizebox{\columnwidth}{!}{\begin{tabular}{c | c c |  c c} \Xhline{2\arrayrulewidth}
%             \textbf{Target Dataset} &  \multicolumn{2}{c|}{BART} &  \multicolumn{2}{c}{BART-arg}  \\
%               &  Relevance & Consistency & Relevance & Consistency \\
%           \Xhline{2\arrayrulewidth} 
%           Reddit   &  3.39 & 3.40 &  3.47 &  3.41 \\
%           AMI   &  4.07 & 3.67 &  4.13 &  3.70 \\
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Relevance and factual consistency annotations for BART and BART-arg outputs on Reddit and AMI.}
% \label{tab:table_human_evaluation}
% \end{table}
% }



% \newcommand{\BARTBenchmarkOthers}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{c c c}
% \Xhline{2\arrayrulewidth}
%              \textbf{Dataset/Method} & Our results  &  Previous SOTA \\  \hline
%             SAMSum & \textbf{52.27/27.82/47.92} & 49.30/25.60/47.70   \\ \hline   
%             CQASUMM  & \textbf{32.79/6.68/28.83} & 31.00/5.00/15.20   \\ \hline  
%             BC3 & 39.59/13.98/21.20 & -   \\ \hline  
%             ADS & 37.18/11.42/21.27 & -   \\ \hline  
%             SENSEI & 34.57/7.08/16.80 & -   \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Benchmarking results on conversational datasets such as SAMSum \cite{gliwa-etal-2019-samsum} and CQASUMM \cite{chowdhury2018cqasumm} and initial neural abstractive summarization results for email (BC3) \cite{JanAAAI08}, debate discussion forums (ADS) \cite{misra-etal-2015-argumentative-dialogue-corpus}, and news comments (SENSEI) \cite{barker2016sensei}.}
% \label{tab:benchmark_others}
% \end{table}
% }



% \newcommand{\ExampleSummariesFirst}{
% \begin{table}[t!]
% \centering
% \small
% \begin{tabularx}{\columnwidth}{|X|}
% \hline
% \textbf{Title}: What should I draw next?   \textbf{Subreddit}: pokemon \\ \hline
%  A FB user said they wanted to see a Zapdos, but depending on what people say on here, if any, I may do one that you all choose! So help out if you want!  Or don't. :) \\ \hline
% \textbf{Source Documents:} \\
%  1.  I'd like to see any of the Legendary Beasts, Raikou, Suicune, Entei. \\
%  2.  Ooo I'm kinda thinking of Suicune now. Good choice! I'll consider it for sure! If not, it will definitely be very soon!    \\
% 3.   Pancham   $\leftarrow$ Oooo good choice. That'll be one of the next ones too.   \\
% 4.   If you have the time, I'd love to see Reshiram!  $\leftarrow$ I'll definitely do that as one of the next ones!  Thank you very much! \\ 
% 5.   Seel?  $\leftarrow$ With your username, I may just do that soon.  $\leftarrow$  Cool!    \\
% 6.   MAGIKARP   $\leftarrow$ Dear Lord. \\
% 7.  Aron & lairon!  \\
% 8.   You should girafarig because it's the best pokemon ever created no matter what ANYONE SAYS.   $\leftarrow$ While I admire your steadfast courage in how awesome Girafig is, I may wait on that one. :P BUT. Maybe. :) \\ \hline
% \textbf{BART:} Most commenters say that they would like to see a Zapdos or Suicune. A few other suggestions are Girafig, Arron, lairon, Magikarp, Raikou, Entei, Reshiram, Seel, and Pancham. One commenter says that they want to see Girafarig, but another says that he may wait on that one for a while. \\ \hline
% \textbf{BART-arg:} Most commenters say that they would like to see a Zapdos, Raikou, Suicune, Entei, Pancham Aron, and lairon. A few commenters say they would love to see Girafarig. One commenter says that he would like Girafig because it's the best pokemon ever created no matter what anyone says about it. Another commenter says they want to see Reshiram. \\ \hline
%  \textbf{Gold Summary:} Commenters suggest ideas of the next Pokemon for the original poster to draw next. Each commenter has a different suggestion including Raikou, Reshiram, Seel, Magikarp and Lairon, and the original poster comments their thoughts on each of the suggestions with either approval or a joking disapproval. \\ \hline
% \end{tabularx}
% \caption{Example source documents and summaries from Reddit data in which the models are faithful to the source and largely relevant.}
% \label{tab:example_summaries_first}
% \end{table}
% }







% \newcommand{\ExampleSummariesSecond}{
% \begin{table}[t!]
% \centering
% \small
% \begin{tabularx}{\columnwidth}{|X|}
% \hline
% \textbf{Title}:  Complete noob here. Any advice welcome!   \textbf{Subreddit}: personalfinance \\ \hline
% I've always been responsible when it comes to my money. In the sense that I dont spend what I dont have, I save my money, and I watch what I spend. But now I've recently graduated (with 28k in debt) and want to do better. I've got, what I think, is a decent plan to pay off my debt. ... But what else should I be doing? ... \\ \hline
% \textbf{Source Documents:} \\ \hline
% 1. Please read the information found in the [FAQ](http://www.reddit.com/r/personalfinance/wiki/faq), particularly ...  \\
% 2. Make sure any extra money is going towards the principal. \\
% 3. If it makes you feel better there was never a class where this was explained. ... The best way to learn is to check out the FAQs on the sidebar ... \\
% 4. ... You should also save up some cash in a bank account and consider that your emergency fund,... \\
% 5. The two common retirement accounts are 401ks and IRAs  \\
% 6. Invest in pumpkins. \\ \hline
% \textbf{BART:} Most commenters agree that the best way to learn about investing is to read the FAQ. A few commenters say that if you have debt, then you should start making contributions to a 401k retirement plan. \textcolor{red}{One commenter says that you need to start a small business to pay off your debt}, and another says that it would be a good idea to have some cash in a bank account. \textcolor{red}{One commentator says that they think the best thing to do is start a business.}  \\ \hline
% \textbf{BART-arg:} Most commenters agree that the best way to start a small business is to pay off your debt. \textcolor{red}{Some commenters} say that you should also invest in pumpkins. One commenter says that if you don’t have a 401k, then you should start making contributions to a Roth retirement plan. Another commenter suggests that you invest in a bank account to build up an emergency fund. One commentator says that you need to be responsible when it comes to your money. \\ \hline
% \textbf{Gold Summary:} Commenters offer their advice for settling a debt. Several commenters agree that utilizing the avalanche model is the correct way to pay the debt. Another also suggests having an emergency fund for any unexpected bills or necessary expenses. In understanding finance, commenters stress the need to check the sidebar for FAQs.  \\ \hline
% \end{tabularx}
% \caption{Example source documents and summaries from Reddit data in which the models fail to completely capture salience while remaining faithful to the input.}
% \label{tab:example_summaries_second}
% \end{table}
% }




==> old/0-save_helpers_sep.tex <==


% % Section 1
% \newcommand{\IntroductionMotivatingExample}{
% \begin{table}[t!]
% \centering
% \small
% \begin{tabularx}{\columnwidth}{|X|}
% \hline
% \textbf{Headline:} SuperBowl
%  \\ \hline
% \textbf{Snippet:} Whether you’re a football fan or not, what do you like about Super Bowl Sunday?
%  \\ \hline
% \textbf{Comment:} ... In my opinion I think the Falcons will stomp the patriots. I think Tom Brady will choke the Super Bowl. ...
% \\ \hline
% \textbf{Comment:}  I am big Arizona Cardinals fan so when they didn't even make the playoffs i was upset. ...
% \\ \hline
% \textbf{Comment:} I'm not a very big football fan at all. So when it comes to Superbowl Sunday, I'm in it for the commercials and the half time show. ...
% \\ \hline
% \textbf{Comment:}  I am not exactly a football fan, but I enjoy watching the Super Bowl....
% \\ \hline
% \textbf{...}
% \\ \hline
% \textbf{Summary:} \\ 
% Several commenters list their favorite things about the Super Bowl, including half-time shows, the funny commercials, the Puppy Bowl, eating food, and spending time with family. A couple of commenters admit to not being football fans but still enjoying the Super Bowl. Some commenters discuss whether they thought the Falcons or the Patriots were going to win, while others list teams they wish were in the game.
%  \\
% \hline
% \end{tabularx}
% \caption{Example summary of comments from a New York Times article discussing people's favorite parts of the Super Bowl. The summary is an analysis of the comments and quantifies the viewpoints present.}
% \label{tab:example}
% \end{table}
% }

% % Section 3
% \newcommand{\DatasetComparison}{
%  \begin{table*}[t!]
% \resizebox{\textwidth}{!}{\begin{tabular}{| c | c c c | c c c | c | c | c | }
% \Xhline{2\arrayrulewidth}
%              \textbf{Dataset} & \multicolumn{3}{c|}{\textbf{\% novel n-grams}} &  \multicolumn{3}{c|}{\textbf{Extractive Oracle}}  &  \textbf{Summary Length} & \textbf{Input Length}  & \textbf{\# Docs/Example} \\  \hline
%             NYT & 36.11 & 79.72 & 94.52 & 36.26 & 10.21 & 31.23 & 79 & 1624 & 16.95  \\ \hline  
%             Reddit & 43.84 & 84.98 & 95.65 & 35.74 & 10.45 & 30.74  & 65 & 641 & 7.88 \\ \hline  
%             Stack & 35.12 & 77.91 & 93.56 &  37.30 & 10.70 & 31.93  & 73 & 1207 & 9.72   \\ \hline  
%             Email & 42.09 & 83.27 & 93.98 & 40.98 & 15.50 & 35.22  & 74 & 917 & 4.95  \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Statistics across dataset sources in ConvoSumm, showing novel uni/bi/tri-grams, ROUGE-1/2/L extractive oracle scores, the average input and summary lengths (number of tokens), as well as the number of documents per example, where each comment/post/answer/email is considered a document.}
% \label{tab:statistics}
% \end{table*}
% }
% \newcommand{\DatasetComparisonMDS}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{| c |  c | c | c c c | }
% \Xhline{2\arrayrulewidth}
%              \textbf{Data/Method} & \textbf{Inter-document Similarity} & \textbf{Redundancy} & \multicolumn{3}{c|}{\textbf{Layout Bias}} \\  \hline
%             NYT & -11.71 & -0.23 & 0.2 & 0.5 & 0.3  \\ \hline  
%             Reddit & -7.56 & -0.49 & 0.2 & 0.5 & 0.2  \\ \hline  
%             Stack & -9.59 & -0.27 & 0.2 & 0.3 & 0.4 \\ \hline  
%             Email & -1.76 & -0.18 & 0.3 & 0.4 & 0.3 \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Multi-document summarization-specific dataset analysis on our proposed datasets with metrics introduced in \citet{dey2020corpora}:   inter-document similarity (father from zero is less similarity), redundancy (father from zero is less overall redundancy of semantic units), and start/middle/end layout bias.}
% \label{tab:statistics_mds}
% \end{table}
% }
% \newcommand{\BaselineResults}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{ | c |  c c c | c c c | c c c |}
% \Xhline{2\arrayrulewidth}
%              \textbf{Data/Method} & \multicolumn{3}{c|}{\textbf{Lexrank}} &  \multicolumn{3}{c|}{\textbf{Textrank}} & \multicolumn{3}{c|}{\textbf{BERT-ext}} \\  \hline
%             NYT & 22.30 & 3.87 & 19.14 & 25.11 & 3.75 & 20.61 & 25.88 & 3.81 & 22.00  \\ \hline  
%             Reddit & 22.71 & 4.52 & 19.38 & 24.38 & 4.54 & 19.84 & 24.51 & 4.18 & 20.95 \\ \hline  
%             Stack & 26.30 & 5.62 & 22.27 & 25.43 & 4.40 & 20.58 & 26.84 & 4.63 & 22.85 \\ \hline  
%             Email & 16.04 & 3.68 & 13.38 & 19.50 & 3.90 & 16.18 & 25.46 & 6.17 & 21.73 \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{ROUGE-1/2/L results for extractive LexRank \cite{erkan2004lexrank}, TextRank \cite{mihalcea2004textrank}, and BERT-based \cite{miller2019leveraging} models.}
% \label{tab:extractive_baselines}
% \end{table}
% }


% % Section 4
% \newcommand{\ArgumentGraph}{
% \begin{figure*}[t!]
%     \centering
%     \includegraphics[scale=0.40]{plots/argument_graph.png}
%     \caption{Sample argument subgraph construct from NYT news comments illustrating varying viewpoints. Claims ``I honestly..." and ``but I dont.." are entailed by premises, connected through \texttt{Default Inference} nodes, and opposing claims are connected through \texttt{Issue} nodes.
%     }
%     \label{fig:argument_graph}
% \end{figure*} 
% }


% % Section 5
% \newcommand{\BARTTransferResults}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{| c |  c c c |  c c c |}
% \Xhline{2\arrayrulewidth}
%              \textbf{Data/Method}  &  \multicolumn{3}{c|}{\textbf{BART}} & \multicolumn{3}{c|}{\textbf{BART-arg}} \\  \hline
%             NYT &  35.91 & 9.22 & 31.28 & \textbf{36.60} & \textbf{9.83} & \textbf{32.61} \\ \hline  
%             Reddit &  35.50 & 10.64 & 32.57 & \textbf{36.39} & \textbf{11.38} &  \textbf{33.57}  \\ \hline  
%             Stack &  39.61 & 10.98 & 35.35 & \textbf{39.73} &  \textbf{11.17} &  \textbf{35.52}  \\ \hline  
%             Email &  \textbf{41.46} &  \textbf{13.76} & \textbf{37.70} & 40.91 & 13.67 & 37.10   \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{ROUGE-1/2/L results for vanilla BART as well as one trained on argument-mining input. Both are trained on 200 points from the ConvoSumm.}
% \label{tab:bart_transfer}
% \end{table}
% }


% % Section 6
% \newcommand{\BARTMeetingResults}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{| c | c c c | c c c | c c c | c c c| }
% \Xhline{2\arrayrulewidth}
%              \textbf{Data/Method} & \multicolumn{3}{c|}{\textbf{HMNet}}  &  \multicolumn{3}{c|}{\textbf{DDA-GCN}}  &  \multicolumn{3}{c|}{\textbf{Longformer-BART}} & \multicolumn{3}{c|}{\textbf{Longformer-BART-arg}} \\  \hline
%             AMI &  53.02 & 18.57 & - & 53.15 & \textbf{22.32} & - & 54.20 & 20.72 & 51.36   &  \textbf{54.47} & 20.83 & \textbf{51.74} \\ \hline  
%             ICSI & \textbf{46.28} & 10.60 & - & & - &  & 43.03 & \textbf{12.14} & 40.26 & 44.17 & 11.69 & \textbf{41.33}  \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{ROUGE-1/2/L results for DDA-GCN \cite{feng2020dialogue} and HMNet \cite{zhu2020a} on the AMI and ICSI meeting summarization dataset along with our Longformer and Longformer-arg models.}
% \label{tab:meeting}
% \end{table}
% }

% \newcommand{\TableHumanEvaluation}{
% \begin{table}[t!]
% \centering
% \resizebox{\columnwidth}{!}{\begin{tabular}{| c | c c |  c c| } \Xhline{2\arrayrulewidth}
%             \textbf{Target Dataset} &  \multicolumn{2}{c|}{BART} &  \multicolumn{2}{c|}{BART-arg}  \\
%               &  Relevance & Consistency & Relevance & Consistency \\
%           \Xhline{2\arrayrulewidth} 
%           Reddit   &  3.39 (0.13) & 3.40 (0.12) &  3.47 (0.12) &  3.41 (0.10) \\
%           AMI   &  4.07 (0.16) & 3.67 (0.16) &  4.13 (0.17) &  3.70 (0.17) \\
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Mean relevance and factual consistency annotations for BART and BART-arg outputs on Reddit and AMI. Standard errors are reported in parentheses.}
% \label{tab:table_human_evaluation}
% \end{table}
% }



% \newcommand{\BARTBenchmarkOthers}{
%  \begin{table}[t]
% \resizebox{\columnwidth}{!}{\begin{tabular}{| c |  c c c |  c c c | }
% \Xhline{2\arrayrulewidth}
%              \textbf{Data/Method} & \multicolumn{3}{c|}{Our results}  &  \multicolumn{3}{c|}{Previous SOTA} \\  \hline
%             SAMSum & \textbf{52.27} & \textbf{27.82} & \textbf{47.92} & 49.30 & 25.60 & 47.70   \\ \hline   
%             CQASUMM  & \textbf{32.79} & \textbf{6.68} & \textb{28.83} & 31.00 & 5.00 & 15.20   \\ \hline  
%             BC3 & 39.59 & 13.98 & 21.20 & & -  &  \\ \hline  
%             ADS & 37.18 & 11.42 & 21.27 & & -  &  \\ \hline  
%             SENSEI & 34.57 & 7.08 & 16.80 & & - &    \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Benchmarking results on conversational datasets such as SAMSum \cite{gliwa-etal-2019-samsum} and CQASUMM \cite{chowdhury2018cqasumm} and initial neural abstractive summarization results for email (BC3) \cite{JanAAAI08}, debate discussion forums (ADS) \cite{misra-etal-2015-argumentative-dialogue-corpus}, and news comments (SENSEI) \cite{barker2016sensei}.}
% \label{tab:benchmark_others}
% \end{table}
% }



% \newcommand{\ExampleSummariesFirst}{
% \begin{table}[t!]
% % \centering
% \small
% \begin{tabularx}{\columnwidth}{|X|}
% \hline
% \textbf{Title}: What should I draw next?   \textbf{Subreddit}: pokemon \\ \hline
%  A FB user said they wanted to see a Zapdos, but depending on what people say on here, if any, I may do one that you all choose! So help out if you want!  Or don't. :) \\ \hline
% \textbf{Source Documents:} \\
%  1.  I'd like to see any of the Legendary Beasts, Raikou, Suicune, Entei. \\
%  2.  Ooo I'm kinda thinking of Suicune now. Good choice! I'll consider it for sure! If not, it will definitely be very soon!    \\
% 3.   Pancham   $\leftarrow$ Oooo good choice. That'll be one of the next ones too.   \\
% 4.   If you have the time, I'd love to see Reshiram!  $\leftarrow$ I'll definitely do that as one of the next ones!  Thank you very much! \\ 
% 5.   Seel?  $\leftarrow$ With your username, I may just do that soon.  $\leftarrow$  Cool!    \\
% 6.   MAGIKARP   $\leftarrow$ Dear Lord. \\
% 7.  Aron & lairon!  \\
% 8.   You should girafarig because it's the best pokemon ever created no matter what ANYONE SAYS.   $\leftarrow$ While I admire your steadfast courage in how awesome Girafig is, I may wait on that one. :P BUT. Maybe. :) \\ \hline
% \textbf{BART:} Most commenters say that they would like to see a Zapdos or Suicune. A few other suggestions are Girafig, Arron, lairon, Magikarp, Raikou, Entei, Reshiram, Seel, and Pancham. One commenter says that they want to see Girafarig, but another says that he may wait on that one for a while. \\ \hline
% \textbf{BART-arg:} Most commenters say that they would like to see a Zapdos, Raikou, Suicune, Entei, Pancham Aron, and lairon. A few commenters say they would love to see Girafarig. One commenter says that he would like Girafig because it's the best pokemon ever created no matter what anyone says about it. Another commenter says they want to see Reshiram. \\ \hline
%  \textbf{Gold Summary:} Commenters suggest ideas of the next Pokemon for the original poster to draw next. Each commenter has a different suggestion including Raikou, Reshiram, Seel, Magikarp and Lairon, and the original poster comments their thoughts on each of the suggestions with either approval or a joking disapproval. \\ \hline
% \end{tabularx}
% \caption{Example source documents and summaries from Reddit data in which the models are faithful to the source and largely relevant.}
% \label{tab:example_summaries_first}
% \end{table}
% }







% \newcommand{\ExampleSummariesSecond}{
% \begin{table}[t!]
% \centering
% \small
% \begin{tabularx}{\columnwidth}{|X|}
% \hline
% \textbf{Title}:  Complete noob here. Any advice welcome!   \textbf{Subreddit}: personalfinance \\ \hline
% I've always been responsible when it comes to my money. In the sense that I dont spend what I dont have, I save my money, and I watch what I spend. But now I've recently graduated (with 28k in debt) and want to do better. I've got, what I think, is a decent plan to pay off my debt. ... But what else should I be doing? ... \\ \hline
% \textbf{Source Documents:} \\ \hline
% 1. Please read the information found in the [FAQ](http://www.reddit.com/r/personalfinance/wiki/faq), particularly ...  \\
% 2. Make sure any extra money is going towards the principal. \\
% 3. If it makes you feel better there was never a class where this was explained. ... The best way to learn is to check out the FAQs on the sidebar ... \\
% 4. ... You should also save up some cash in a bank account and consider that your emergency fund,... \\
% 5. The two common retirement accounts are 401ks and IRAs  \\
% 6. Invest in pumpkins. \\ \hline
% \textbf{BART:} Most commenters agree that the best way to learn about investing is to read the FAQ. A few commenters say that if you have debt, then you should start making contributions to a 401k retirement plan. \textcolor{red}{One commenter says that you need to start a small business to pay off your debt}, and another says that it would be a good idea to have some cash in a bank account. \textcolor{red}{One commentator says that they think the best thing to do is start a business.}  \\ \hline
% \textbf{BART-arg:} Most commenters agree that the best way to start a small business is to pay off your debt. \textcolor{red}{Some commenters} say that you should also invest in pumpkins. One commenter says that if you don’t have a 401k, then you should start making contributions to a Roth retirement plan. Another commenter suggests that you invest in a bank account to build up an emergency fund. One commentator says that you need to be responsible when it comes to your money. \\ \hline
% \textbf{Gold Summary:} Commenters offer their advice for settling a debt. Several commenters agree that utilizing the avalanche model is the correct way to pay the debt. Another also suggests having an emergency fund for any unexpected bills or necessary expenses. In understanding finance, commenters stress the need to check the sidebar for FAQs.  \\ \hline
% \end{tabularx}
% \caption{Example source documents and summaries from Reddit data in which the models fail to completely capture salience while remaining faithful to the input.}
% \label{tab:example_summaries_second}
% \end{table}
% }






% \newcommand{\BARTTransferFullResults}{
%  \begin{table}[h!]
% \resizebox{\columnwidth}{!}{\begin{tabular}{| c |  c c c |  c c c | c c c | }
% \Xhline{2\arrayrulewidth}
%              \textbf{Data/Method}  &  \multicolumn{3}{c|}{\textbf{BART}} & \multicolumn{3}{c|}{\textbf{BART-arg-graph}} & \multicolumn{3}{c|}{\textbf{BART-arg-filtered}}\\  \hline
%             NYT &  35.91 & 9.22 & 31.28 & 36.02 & 9.60 &  32.34 & \textbf{36.60} & \textbf{9.83} & \textbf{32.61} \\ \hline  
%             Reddit &  35.50 & 10.64 & 32.57 & 36.39 & \textbf{11.38} &  \textbf{33.57} &  \textbf{36.51} & 11.02 & 33.14 \\ \hline  
%             Stack &  39.61 & 10.98 & 35.35 & \textbf{39.73} &  \textbf{11.17} &  \textbf{35.52} & 39.40 & 10.98 & 35.51 \\ \hline  
%             Email &  \textbf{41.46} &  \textbf{13.76} & \textbf{37.70} & 39.05 & 12.14 & 35.99 & 40.91 & 13.67 & 37.10  \\ \hline  
%             \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{ROUGE-1/2/L results for vanilla BART as well as one trained on argument-mining input. Both are trained on 200 points from the ConvoSumm.}
% \label{tab:bart_transfer_full}
% \end{table}
% }



==> old/prev.tex <==
% Related work
% \textbf{Modeling Conversational Summarization:}
%  Early approaches to conversation summarization consisted of feature engineering \citep{xie2008feature}, template selection methods \citep{oya-etal-2014-template}, and statistical machine learning approaches \citep{galley-2006-skip, wang-cardie-2013-domain}. More recent modeling approaches for dialogue summarization have attempted to take advantage of conversation structures found within the data through dialogue act classification, discourse labeling, and topic segmentation. \citet{goo-2018-abstractive} leveraged \textit{dialogue act} information, which describes the effect of an utterance on its context as an interactive signal, e.g., “assess,” “inform,” “suggest,” to jointly train with the summarization model. \citet{ganesh-2019-abstractive} further use discourse labels to restructure the entire conversation into a single document and then apply any off-the-shelf document summarization method, effectively working in zero-shot settings. Since key information about specific topics is often scattered across multiple utterances within a conversation, \citet{liu-2019-topic} conducted \textit{topic segmentation} using a Pointer-Generator network \citep{see-etal-2017-get} to combat the effect of topic diffusion and intra-utterance topic drift. To handle the same issue, \citet{liu-2019-automatic} maintained \textit{key point sequences} as auxiliary labels that help the summarization model learn the logic of the summary, thus improving their logic, integrity, and correctness. In a more holistic approach, \citet{chen2020multiview} utilized multiple conversational structures from different perspectives in its sequence-to-sequence model, including the topic, stage, global and discrete views of the conversation. However, such approaches focus on dialogue summarization, and it is not trivial to extend such methods to longer conversations with many more participants. We thus introduce a method to model the structure of the discourse over the multi-party conversation. 
